On student-teacher deviations in distillation: does it pay to disobey?

Knowledge distillation (KD) has been widely used to improve the test accuracy of a "student" network, by training it to mimic the soft probabilities of a trained "teacher" network. Yet, it has been shown in recent work that, despite being trained to fit the teacher's probabilities, the student may not only significantly deviate from the teacher probabilities, but may also outdo than the teacher in performance. Our work aims to reconcile this seemingly paradoxical observation. Specifically, we characterize the precise nature of the student-teacher deviations, and argue how they can co-occur with better generalization. First, through experiments on image and language data, we identify that these probability deviations correspond to the student systematically exaggerating the confidence levels of the teacher. Next, we theoretically and empirically establish another form of exaggeration in some simple settings: KD exaggerates the implicit bias of gradient descent in converging faster along the top eigendirections of the data. Finally, we tie these two observations together: we demonstrate that the exaggerated bias of KD can simultaneously result in both (a) the exaggeration of confidence and (b) the improved generalization of the student, thus offering a resolution to the apparent paradox. Our analysis brings existing theory and practice closer by considering the role of gradient descent in KD and by demonstrating the exaggerated bias effect in both theoretical and empirical settings.

==> switching.tex <==
\subsection{Which deviations matter: A study of loss-switching}
\label{sec:switching}

\textbf{Motivation.} Another kind of student-teacher deviation that prior work has looked at are deviations in the training trajectory that emerge very early on during neural network training: these deviations perhaps condition 
 the network into a more favorable representation \cite{zhu20towards} or a basin in the non-convex loss ~\citep{jha20demystification}.
In this section, we examine the relevance of these early-phase deviations to the gains of distillation, and also on the probability deviations observed in the previous section.








\textbf{Experiment design.} To test the relevance of early-phase deviations, we propose {\em late distillation} where we train a network with one-hot loss for a fair part (say, half) of training, and then switch to distillation loss. If distillation relied crucially on early-phase deviations, late distillation should \textit{not} result in substantial improvements over one-hot training.


    
\begin{figure*}[!t]
\centering
\subfloat[One-hot and self-distillation.]{\label{fig:logit-evolution-oh-kd}
\begin{tabular}[b]{@{}c@{}}
\adjincludegraphics[width=.5\linewidth,trim= 0 0 0 2em, clip=true]{Images/cf100.res56.res56.train_all/standalone_scatter_inv-t-probs_-1_train_all.png}\\[-3pt]
\adjincludegraphics[width=.5\linewidth,trim= 0 0 0 2em, clip=true]{Images/cf100.res56.res56.train_all/student_scatter_inv-t-probs_-1_train_all.png}%
\end{tabular}%
}
\subfloat[Loss-switching to distillation/one-hot at $15k$ steps.]{\label{fig:logit-evolution-loss-switching}
\begin{tabular}[b]{@{}c@{}}
\includegraphics[width=.5\linewidth,trim= 0 0 0 2em, clip=true]{Images/cf100.res56.res56.train_all/distill_from_15000_scatter_inv-t-probs_-1_train_all.png}\\[-3pt]
\includegraphics[width=.5\linewidth,trim= 0 0 0 2em, clip=true]{Images/cf100.res56.res56.train_all/onehot_from_15000_scatter_inv-t-probs_-1_train_all.png}%
\end{tabular}%
}
    \caption{\textbf{Evolution of teacher-student logit plots over various steps of training for CIFAR100 ResNet56 self-distillation setup:} On the \textbf{left}, we present plots for one-hot training (\textbf{top}) and distillation (\textbf{bottom}). %
    On the \textbf{right}, we present similar plots for experiments from Section~\ref{sec:switching}, with the loss switched to distillation (\textbf{top}) and one-hot (\textbf{bottom}) at $15k$ steps. From the last two  plots in these two, we find that switching to distillation ``unlearns'' low-confidence points, while switching to one-hot ``{fixes}'' the underfitting.
    }
    \label{fig:logit-evolution}
\end{figure*}

    
    
    
\textbf{Observations.} We make three key observations here. First, from Figures~\ref{fig:train-switching-plots} (and \S\ref{app:loss-switching} Fig~\ref{fig:late-distillation-appendix}),
we observe that replacing the first $1/4$th of training with one-hot is able to recover \textit{all} of distillation's gains in our CIFAR100 and TinyImagenet settings; replacing the first $1/2$ of training, recovers a signifcant fraction of the gains. This happens despite the fact that when we switch to distillation, we  have a much smaller learning rate (due to our chosen schedule, see \S\ref{app:hyperparameters}). For CIFAR100 in particular, we are able to begin self-distillation even after 95\% of training is complete, and still expect to see strong gains. This implies that {\em early phase deviations are not as critical for distillation to help} as previously thought.

Conversely, we also switch from distillation to one-hot in Fig~\ref{fig:intro-loss-switching} and Fig~\ref{fig:loss-switching-tinyin}. Here we find that switching to one-hot {\em undoes} a considerable fraction of the gains that distillation has achieved thus far, given a sufficiently long one-hot training. {\em This suggests an inherent destructive effect in one-hot gradients} that we formalize in \S\ref{sec:gradient-space-view}. We provide a more nuanced discussion of these experiments in \S\ref{app:loss-switching} (and Fig~\ref{fig:late-onehot-appendix}) of interest to practitioners.\footnote{Note that switching to one-hot does not as aggressively undo the gains of distillation when compared to the converse scenario where a switch to distillation aggressively improves over one-hot training.}


For our final observation, we examine how the underfitting behavior of distillation evolves under loss-switching. In Fig~\ref{fig:logit-evolution-loss-switching}, we plot a series of scatter plots in the style of 
 \S\ref{sec:margin-per-sample}, where the $X$ axis is the teacher's final top class probability on a point, and the $Y$ axis is the student's probability {\em taken as a snapshot at some intermediate timestep}. Here, we find that even though early-phase one-hot training has already fit all examples to a certain extent, we surprisingly find that a subsequent switch to distillation  ``unlearns'' the low-confidence examples to force the typical underfitting behavior from  \S\ref{sec:margin-per-sample}. Conversely, switching to one-hot {\em fixes} the underfitting induced by an initial distillation phase.  
 


In summary, we argue that these experiments emphasize that the underfitting phenomenon from \S\ref{sec:margin-per-sample} must be fundamental to the behavior of distillation, while early-phase student-teacher deviations are not critical. 










As a final note, we find that in both CIFAR100 (Fig~\ref{fig:interp-cifar100}) and TinyImageNet (\S\ref{app:loss-switching}), switching the other way, {\em from} one-hot {\em to} distillation, late during training is sufficient to induce an exaggeration of confidence levels. In fact, we also find a simultaneous increase in accuracy accompanied with the switch. This implies that at least in these settings, the regularization effect of distillation  can occur even at a ``superficial stage'' of the training process, in contrast to other proposed effects of distillation such as feature-learning \citep{zhu20towards} or conditioning towards a different basin \cite{jha20demystification} which must happen only early during training.
